Online Stabilization of Unknown Linear Time-Varying Systems

This paper studies the problem of online stabilization of an unknown discrete-time linear time-varying (LTV) system under bounded non-stochastic (potentially adversarial) disturbances. We propose a novel control algorithm based on convex body chasing (CBC). Under the assumption of infrequently changing or slowly drifting dynamics, the algorithm guarantees bounded-input-bounded-output stability in the closed loop. Our approach avoids system identification and applies, with minimal disturbance assumptions, to a variety of LTV systems of practical importance. We demonstrate the algorithm numerically on examples of LTV systems including Markov linear jump systems with finitely many jumps.

==> preamble.tex <==
\usepackage{mathptmx}
\usepackage[libertine]{newtxmath}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsfonts}
% \usepackage{bbm}
% \usepackage{amssymb}
% \usepackage{amstext}
\usepackage{thmtools}
\usepackage{theorem}
\usepackage{comment}
\usepackage{xcolor}
% \usepackage{multirow}
\usepackage{comment}
% \usepackage{amssymb,amsmath,amsthm}
% \usepackage[pagebackref=true]{hyperref}
\usepackage{mathtools}
% \let\Bbbk\relax % to solve the incompatible between amssymb & acmart(containing newtxmath)


\usepackage{dsfont}
\usepackage[vlined,ruled,resetcount]{algorithm2e}
\usepackage[hidelinks]{hyperref}
\usepackage{cleveref}

\usepackage[usestackEOL]{stackengine}
\def\dashint{\,\ThisStyle{\ensurestackMath{%
  \stackinset{c}{.2\LMpt}{c}{.5\LMpt}{\SavedStyle-}{\SavedStyle\phantom{\int}}}%
  \setbox0=\hbox{$\SavedStyle\int\,$}\kern-\wd0}\int}

\allowdisplaybreaks

%%% Varun Commands
\newcommand{\Fbar}{\bar{F}} % Loss
\newcommand{\stab}{\textsf{stab}}
\newcommand{\st}{\textsf{st}}
\newcommand{\bias}{\textsf{bias}}
\newcommand{\var}{\textsf{var}}
\newcommand{\bad}{\textsf{bad}}
\newcommand{\RR}{\mathbb{R}}
\newcommand\abs[1]{\left|#1\right|}
\newcommand\norm[1]{\left\Vert#1\right\Vert}
\newcommand\infnorm[1]{\left\Vert#1\right\Vert_\infty}
\def\cI{{\mathcal{I}}}
\def\cJ{{\mathcal{J}}}
\newcommand{\cW}{\mathcal{W}}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator



\newcommand{\dlyap}{\textsf{dlyap}}

\let\hat\widehat
\let\tilde\widetilde
\let\check\widecheck
\def\given{{\,|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}

%%% Jing Commands
\newcommand{\OPT}[1]{\textsc{OPT}_{[0,#1]}}
\newcommand{\INT}[1]{\textsc{INT}_{[0,#1]}}
\newcommand{\sysm}{\{\theta_t\}_{t=0}^{\infty}} % time-carying system matrices
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\indicator}[1]{\mathds{1}_{#1}}
\newcommand{\tr}{\mbox{Tr}\,}
\usepackage{scalerel}
\usepackage[usestackEOL]{stackengine}

\newcommand{\approxtext}[1]{\ensuremath{\stackrel{\text{#1}}{\approx}}}

\def\dashint{\,\ThisStyle{\ensurestackMath{%
            \stackinset{c}{.2\LMpt}{c}{.5\LMpt}{\SavedStyle-}{\SavedStyle\phantom{\int}}}%
        \setbox0=\hbox{$\SavedStyle\int\,$}\kern-\wd0}\int}

\newcommand{\dINT}[2]{\Delta^{\textsc{INT}}_{[#1,#2]} }
\newcommand{\dOPT}[2]{\Delta^{\textsc{OPT}}_{[#1,#2]} }

\makeatletter
\newcommand{\changeoperator}[1]{%
  \csletcs{#1@saved}{#1@}%
  \csdef{#1@}{\changed@operator{#1}}%
}
\newcommand{\changed@operator}[1]{%
  \mathop{%
    \mathchoice{\textstyle\csuse{#1@saved}}
               {\csuse{#1@saved}}
               {\csuse{#1@saved}}
               {\csuse{#1@saved}}%
  }%
}
\makeatother

% \changeoperator{sum}
\changeoperator{prod}


%%% Highlight
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}{\color{green}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\adam}[1]{\textcolor{red}{(adam: #1)}}
\newcommand{\varun}[1]{\textcolor{red}{(varun: #1)}}
